Structured Sparsity: Discrete and Convex approaches

Compressive sensing (CS) exploits sparsity to recover sparse or compressible signals from dimensionality reducing, non-adaptive sensing mechanisms. Sparsity is also used to enhance interpretability in machine learning and statistics applications: While the ambient dimension is vast in modern data analysis problems, the relevant information therein typically resides in a much lower dimensional space. However, many solutions proposed nowadays do not leverage the true underlying structure. Recent results in CS extend the simple sparsity idea to more sophisticated {\em structured} sparsity models, which describe the interdependency between the nonzero components of a signal, allowing to increase the interpretability of the results and lead to better recovery performance. In order to better understand the impact of structured sparsity, in this chapter we analyze the connections between the discrete models and their convex relaxations, highlighting their relative advantages. We start with the general group sparse model and then elaborate on two important special cases: the dispersive and the hierarchical models. For each, we present the models in their discrete nature, discuss how to solve the ensuing discrete problems and then describe convex relaxations. We also consider more general structures as defined by set functions and present their convex proxies. Further, we discuss efficient optimization solutions for structured sparsity problems and illustrate structured sparsity in action via three applications.

==> clustering_exp.tex <==
\subsection{Clustered image recovery from compressed data}

We compare the performance of 5 clustering priors in recovering a naturally clustered image from its compressive measurements. We take a $m \times m$ image $\x \in \reals^{m^2}$. We try to recover it from $M$ compressive measurements $\y \in \reals^M$ by applying a random Gaussian matrix $A \in reals^{M \times m^2}$ where $a_i \sim \N(0,M)$. Then the measurements are given by $\y= A\x$. We use the following methods to recover $\x$ from $\y$: 
\begin{enumerate}
\item Sparse Ising model \eqref{eq:ising} (IC):
\[ \min \| \y - A\x \|_2^2 + \lambda R_{\text{ISING}}(\supp(\x)) + \tau |\supp(\x)|\]
\item Basis Pursuit (BP):
\[ \min \|\x\|_1 \text{ subject to } \y=A \x \]
\item Total variation (TV) \eqref{def:TV}
\[ \min \|\x\|_1 \text{ subject to } \y=A \x \]
\item Overlapping group Lasso (OGL):
\[ \min \|\x\|_{OGL} \text{ subject to } \y=A \x \]
\end{enumerate}
The Sparse Ising model is solved using the proposed Majorization-Minimization algorithm \ref{sec:sub_discrete}, with the SFM subproblem solved by a maximum flow algorithm. The convex methods are solved using 


==> convex.tex <==
%!TEX root = CS_BOOK_STRUCTSPARSE.tex

\subsection{Convex}

\begin{enumerate}
\item Group-based models and related norms (Group Lasso, Sparse Group Lasso, Overlapping Group Lasso and Latent Group Lasso)
\item Hierarchical structures
\item Generalization I: atomic norms
\item Norms derived from submodular functions (Bach \& Marwa stuff)
\item Generalizations II (My AISTATS paper?)
\end{enumerate}

\subsection{Algorithms}
\begin{enumerate}
\item Proximal methods
\item ADMM

\end{enumerate}

==> discrete.tex <==
%!TEX root = CS_BOOK_STRUCTSPARSE.tex
\section*{Discrete structured sparsity}

%\textcolor{red}{All the rest are under review - feel free to remove/change without notification - references to be included later}
%
%Sparse signal approximation theory lies at the heart of exciting developments in the areas of signal processing and convex/discrete optimization. Sparse signal approximation roughly states that a sparse signal, compared to its ambient dimension, can be perfectly reconstructed from far fewer samples than dictated by the well-known Nyquist-Shannon theorem. 
%According to Shannon-Nyquist sampling theorem, we can perfectly reconstruct $ \xtrue $ by uniformly taking samples with frequency at least twice the highest frequency contained in $ \xtrue $. The true frequency threshold can be easily approximated by applying Fourier tranform on the set of data samples $ \xtrue $.
%Unfortunately, sampling in Shannon-Nyquist rate is prohibitive for computationally demanding real-time applications. Operating at these data rates creates vast amount of data which must be stored, compressed or transmitted. To confront this problem, one has to either use high-end technology infrastructure, increasing the operational cost (higher cost per sample), or reduce the Quality of Service by subsampling. %, i.e., by reducing the amount of data acquired. 
%
%To accomplish this, efficient sparse approximation algorithms have been proposed that tackle phenomena like the ``curse of dimensionality'' with low computational cost, accompanied with strong theoretical convergence and approximation guarantees. During the past two decades, a broad range of applications, from medical imaging and communications to computational biology and microarray data analysis, found practical solutions in sparse signal approximation that reduce the total complexity while maintaining or even improving the solution quality compared to state-of-the-art approaches. 
%
%As our running example, we consider the Compressed Sensing (CS). CS is a data acquisition and recovery technique for finding sparse solutions to linear inverse problems from sub-Nyquist measurements. To accomplish this, CS features a wide range of computationally efficient and robust signal recovery methods, based on sparsity seeking optimization. 
%CS theory is based on the sparse transform coding technique. To describe the main idea, assume $ y \in \mathbb{R}^n $ is a dense $ n $-dimensional vector of interest. Instead of processing $ y $ in its dense representation, the literature today offers 
%%According to Shannon-Nyquist sampling theorem, we can perfectly reconstruct $ \xtrue $ by uniformly taking samples with frequency at least twice the highest frequency contained in $ \xtrue $. %The true frequency threshold can be easily approximated by applying Fourier tranform on the set of data samples $ \xtrue $.
%%Unfortunately, sampling in Shannon-Nyquist rate is prohibitive for computationally demanding real-time applications. Operating at these data rates creates vast amount of data which must be stored, compressed or transmitted. To confront this problem, one has to either use high-end technology infrastructure, increasing the operational cost (higher cost per sample), or reduce the Quality of Service by subsampling. %, i.e., by reducing the amount of data acquired. 
%% The true frequency threshold that defines the time period between consecutive samples in SNWK theorem can be easily approximated by applying Fourier Tranform (FT) on the signal of interest. FT re-represents signals as a weighed sum of complex exponentials in various frequencies. By keeping only the FT coefficients, we can reconstruct the signal by using the inverse FT procedure. But, FT is one of the possible transformations that can be applied to the underlying signal. 
%%Focusing on sparse signal representation, many references in the literature propose 
%signal basis transforms that promote data compression and sparsity. %In more detail, a signal $ \xtrue \in \mathbb{R}^n  $ can be described as a $ k $-sparse linear combination of atoms $ \lbrace \psi_i \rbrace_{i = 1}^{n} $ that correspond to columns of an appropriate basis matrix $ \Psi \in \mathbb{R}^{n \times n} $. 
%Thus, using the appropriate basis matrix\footnote{Most of CS research papers assume the least common case where signals are sparse in an orthonormal basis. In practice, many signals of interest can only be expressed as a linear combination of a few atoms from an {\it overcomplete} dictionary $ D \in \mathbb{R}^{d \times n} $ ($ d > n $) where the columns are correlated. Proving the applicability and efficiency of compressed sensing theory for this general case is part of ongoing research.} $ \Psi \in \mathbb{R}^{n \times n} $, $ y $ can be described as a $ k $-sparse $ (k \ll n) $ linear combination of atoms $ \lbrace \psi_i \rbrace_{i = 1}^{n} $ that correspond to columns of $ \Psi $. This representation can be either exact, $ y = \Psi \xtrue $, or approximate, $ y \approx \Psi \xtrue $, where $ \xtrue \in \mathbb{R}^n $ denotes the set of coefficients with only $ k $ out of $ n $ entries being nonzero. %Typical examples of sparse-inducing bases are wavelet transform for piecewise smooth signals, Fourier transform for smooth signals, curvelets for images with edges, etc. 
%
%Using this key observation, CS proposes an alternative sampling theorem where $ i) $ the sampling process is not periodic, $ ii) $ the samples are acquired through linear projections of the signal of interest with an appropriate measurement matrix and, $ iii) $ the number of measurements needed for signal recovery is much less compared to traditional sampling techniques. 
%
%\subsection{Sparse signal approximation in compressed sensing} 
%
%In the standard CS framework, we reconstruct a high-dimensional signal $ \xtrue \in \mathbb{R}^n $ through a low-dimensional observation vector $ u \in \mathbb{R}^m~(m < n) $ such that:
%\begin{equation}\label{eq:observations}
%  \obs = \sensing \xtrue + n.
%\end{equation} 
%In this setting, $\sensing \in \R^{m\times n}$ represents the measurement/sensing matrix and $ n \in \mathbb{R}^m $ is an additive noise term. For clarity and without loss of generality, we assume that the signal of interest $ \xtrue $ is $ k $-sparse for the rest of the paper, unless otherwise stated.%take $ m \ll n $ measurements $ \obs \in \mathbb{R}^m $ by linearly projecting $ \alpha $ on a measurement matrix $ \Theta \in \mathbf{R}^{m \times n} $, i.e. $ \obs = \Theta \alpha = \Theta \Psi x $. 
%
%To recover $ \xtrue $ given $ \obs $ and $ \sensing $, {\it unconstrained} least-squares method is the classic approach to the solution of linear systems by minimizing the data error function $ f(x) \triangleq \vectornorm{\obs - \sensing \signal}_2^2 $ where $\|\cdot\|_q$ denotes the $\ell_q$-norm. Nevertheless, the reconstruction of $ \xtrue $ from $ u $ is an ill-posed problem since $ m < n $ and there is no hope in finding the {\it true vector} without ambiguity; there is an infinite number of possible solutions that satisfy the linear system of equations. Therefore, additional signal prior knowledge should be exploited by the optimization solver. Using the fact that $ \xtrue $ is $ k $-sparse, we concentrate on the following constrained minimization problem to recover $ \xtrue $: 
%\begin{equation}
%	\begin{aligned}
%	& \underset{x\in\mathbb{R}^n}{\text{minimize}}
%	& & f(x)
%	& \text{subject to}
%	& & \vectornorm{x}_0 \leq k,
%	\end{aligned} \label{opt:00}
%\end{equation} where $ \vectornorm{x}_0 $ is the ``norm'' that counts the non-zero entries in $ x $. %$ \Sigma_k^n $ denotes the union of subspaces in $ n $-dimensions where at most $ k $ out of $ n $ entries are nonzero.
%
%%%%%%%%%%%%%%%%%% !!!!!! footnote -> PMAP ????? %%%%%%%%%%%%%%%%%%%%
%
%%Given the above, the majority of results in CS are based on the following problem formulation: we are interested in finding the sparse solution of the system of equations
%%%\begin{align}
%%%\min_{x: \vectornorm{x}_0 \leq K} \vectornorm{u - \Phi x}^2_2, \label{regr:00}
%%%\end{align}
%%\begin{equation}
%%	\begin{aligned}
%%	& \underset{x}{\text{minimize}}
%%	& & \vectornorm{\obs - \sensing x}^2_2 \\
%%	& \text{subject to}
%%	& & \vectornorm{x}_0 \leq k,
%%	\end{aligned} \label{opt:00}
%%\end{equation}
%% where $ \vectornorm{\cdot}_0 $ is the $ l_0 $-``norm'' that represnents the cardinality of a vector support set. If $ m \geq n $, the above system is overdetermined and there is a closed form solution using the Moore-Penrose pseudoinversion on the sensing matrix $ \sensing $. On the other hand, without assuming any prior information on $ x $, one has no hope on finding a unique solution to this problem when $ m < n $; the system is underdetermined and there is an infinite number of possible solutions $ x $ that satisfy the linear system of equations. 
% 
%%CS theory plays an important role at this point: assuming sparsity constraint in (\ref{opt:00})
%CS theory plays an important role in solving (\ref{opt:00}): assuming signal sparsity, the true solution $ \xtrue $ can be found using $ m \ll n $ measurements, as long as the geometry of sparse signals is preserved after projection on the column subspace defined by $ \sensing $. %\footnote{This idea boils down to the so called restricted isometry property (RIP) with smallest $ k $-th order isometry constant $ \delta_k $ according to which the sensing matrix $ \sensing $ must satsify: 
%%\begin{align}
%%(1 - \delta_k) \leq \frac{\vectornorm{\sensing x}_2^2}{\vectornorm{x}^2_2} \leq (1 + \delta_k), \nonumber
%%\end{align} for any $ x \in \Sigma_k^n $ sparse vector.} 
%%Furthermore, apart from theoretically characterizing the minimum number of measumerents needed to reconstruct the signal of interest, efficient sparse signal recovery algorithms are investigated that find a solution to the above underdetermined system, assuming that $ x $ is a sparse vector, i.e. data in vector $ \alpha $ can be sparsely represented under projection on proper orthonormal basis.
%To achieve this, CS concentrates on developing polynomial-time algorithms for sparse signal recovery from a limited number of non-adaptive samples. Although the collection of works in this direction grows fast, the problem of constructing efficient methods both in execution time and signal recovery performance remains widely open. 
%
%\subsection{Simple sparsity: Two camps of sparse approximation algorithms}
%
%In this subsection, we briefly highlight two major classes of sparse approximation algorithms: $ i) $ the convex optimization approach using interior-point methods and linear programming (LP) solvers and $ ii) $ the class of combinatorial-based greedy algorithms. 
%
%%The family of sparse recovery algorithms can be roughly separated into two major classes: $ i) $ the class of convex optimization solvers and $ ii) $ the greedy-based deterministic algorithms. 
%
%%Convex optimization approach is the one of the first algorithmic efforts for signal approximation in sparse linear inverse problems. 
%In \cite{Chen98atomicdecomposition}, Donoho et. al. demonstrate that, under basic incoherence properties of the sensing matrix $ \sensing $ and given $ \xtrue $ is sufficiently sparse, we can substitute the combinatorial ``norm'' $ \vectornorm{\cdot}_0 $ in (\ref{opt:00}) by its sparsity-inducing convex surrogate $ \vectornorm{\cdot}_1 $ with provable guarantees for unique signal recovery. Using this property, the authors proposed two reformulations of (\ref{opt:00}): the equality-constrained $ l_1 $-norm minimization problem (Basis Pursuit (BP)):
%%\footnote{In the presence of noise, the problem is formulated as
%%\begin{equation*}
%%	\begin{aligned}
%%	& \underset{x}{\text{minimize}}
%%	& & \vectornorm{x}_1 \\
%%	& \text{subject to}
%%	& & \vectornorm{\obs - \sensing x}_2 \leq \vectornorm{e}_2,
%%	\end{aligned} 
%%\end{equation*} where $ e $ is the noise term.
%%}
%\begin{equation}
%	\begin{aligned}
%	& \underset{x\in\mathbb{R}^n}{\text{minimize}}
%	& & \vectornorm{x}_1
%	& \text{subject to}
%	& & \obs = \sensing x,
%	\end{aligned} \label{opt:01}
%\end{equation} for the noiseless case and the regularized optimization problem in the presence of noise (Basis Pursuit DeNoising (BPDN)):
%%%%%%%%%%%%%%%%%%%%% !!! foootnote -> for BPSN use the footnote above %%%%%%%%%%%%%% 
%\begin{equation}
%	\begin{aligned}
%	& \underset{x\in\mathbb{R}^n}{\text{minimize}}
%	& & \frac{1}{2}f(x) + \tau \vectornorm{x}_1,
%	\end{aligned} 
%\end{equation} where $ \tau > 0 $ balances the error norm and the sparsity of the solution. From a different perspective, Tibshirani \cite{tibshirani96regression} proposes the Least Absolute Shrinkage Selection Operator algorithm, dubbed as LASSO:
%\begin{equation}
%	\begin{aligned}
%	& \underset{x\in \mathbb{R}^n}{\text{minimize}}
%	& & f(x)
%	& \text{subject to}
%	& & \vectornorm{x}_1 \leq \lambda,
%	\end{aligned} \label{opt:02}
%\end{equation} where $ \lambda > 0 $ is a regularization parameter that governs the sparsity of the solution.  
%
%Once (\ref{opt:00}) is relaxed to a convex problem, decades of knowledge on convex analysis and optimization can be leveraged. 
%%Since (\ref{opt:01}) can be equivalently reformulated as a linear program [candes], both Linear Programming (LP) solvers and 
%To solve (\ref{opt:01})-(\ref{opt:02}), interior point methods find a solution with fixed precision in polynomial time but their complexity might be prohibitive even for moderate-sized problems. More suitable for large-scale data analysis, fast first-order gradient descent algorithms constitute low-complexity alternatives to these methods; %A major alternative to these methods is based on first-order gradient methods suitable for large-scale data analysis; 
%a non-exhaustive list of examples includes the optimal gradient descent methods proposed by Nesterov \cite{Nesterov00} and the iterative soft thresholding method (IST) \cite{beck2009fast}.
%
%%Characteristic examples of this class are the Basis Pursuit Denoising algorithm \cite{BPDN:00} and the LASSO algorithm \cite{LASSO:00}. The complexity of algorithms falling in this class still remains highly impractical for most of the applications. 
%
%In contrast to the conventional convex relaxation approaches, iterative greedy algorithms maintain the combinatorial nature of (\ref{opt:00}).
%Unfortunately, solving (\ref{opt:00}) with optimality is in general NP-hard and exhaustive search over $ \binom{n}{k} $ possible support configurations of the $ k $-sparse solution is mandatory. Due to this computational intractability, the algorithms of this class greedily refine a $ k $-sparse solution using only ``local'' information available at the current iteration. %from the current $ k $-sparse estimate and the gradient of the objective function at the current iteration. %greedily select indices that maximize the correlation between sensing column vectors and current iteration residual signal $ \obs - \sensing x_i $.\footnote{Also, known as Correlation Maximization (CM) metric \cite{SP:00}.} 
%%The list of algorithms in fastly growing; 
%Representative examples of this class are hard thresholding methods \cite{iht}-\cite{Foucart_hardthresholding} and Matching Pursuit-based algorithms \cite{MallatMP}-\cite{OMP}.
%
%%Representative examples of this class are the hard thresholding methods (Iterative Hard Thresholding (IHT) [], Compressive Sampling Matching Pursuit (CoSaMP) [], Subspace Pursuit (SP) [] and, Hard Thresholding Pursuit (HTP) [] to name a few) and Matching Pursuit-based algorithms (Orthogonal Matching Pursuit (OMP) \cite{OMP:00}, Regularized OMP \cite{ROMP:00},\cite{ROMP:01}, Stagewise OMP \cite{StOMP:00}, etc.)
%
%%In this paper we concentrate on IHT algorithm and prove its relevance to discrete set-function maximization problems. Briefly, hard thresholding algorithm is a popular sparse recovery method, known for its simplicity, ease of implementation, and low computational complexity per iteration. The algorithm can be described only by the following simple recursion: 
%%\begin{align}
%%x_{i+1} = \mathcal{H}_k(x_i + \mu\sensing^T (\obs - \sensing x_i)), \label{eq:00}
%%\end{align} where $ i $ is the iteration count, $ \mathcal{H}_k(\cdot) $ is the projection onto $ k $-sparse signals and $ \mu $ is a step-size quantity.
%%
%%IHT algorithms are exhaustively studied from the perspective of gradient descent optimization under sparsity constraints. In their pure formulation, they were first introduced in a paper by Davies and Blumensath \cite{IHT:00} where, based on Landweber projected regularization method \cite{LAND:00}, they adjusted the algorithm in \cite{LAND:00} to be compatible with general linear inverse problems under sparsity constraints. In parallel, a series of hybrids created like Compressive Sampling Matching Pursuit (CoSaMP) \cite{CoSaMP:00}, Subspace Pursuit (SP) \cite{SP:00}, Hard Thresholding Pursuit (HTP) \cite{HTP:00}, etc.

%\subsection{Structured sparsity}

%\subsubsection{Motivation}

While simple sparsity model is the de facto prior signal information used in many applications, more than that is usually known a-priori. For example, in image processing it is generally known that piecewise smooth signals have sparse wavelet representations where the non-zero coefficients are distributed on a rooted connected tree. Furthermore, block-sparse signals also admit special structure since the signal's support set is clustered into groups; this kind of structure is often found in computational biology and microarray data analysis applications. 

Given additional signal structure information, we construct new combinatorial sparsity models (CSM) to truly make an impact in structured sparsity problems. Some first results are presented in \cite{modelCS} where the authors prove that, under special structures, the number of measurements for successful recovery can be further reduced to $ m = \mathcal{O}(k) $, independent of the ambient signal dimension, $ n $. To extend this work, we present new definitions and results on structured sparsity where the impact of approximating projections on CSM subspaces is mirrored in the convergence guarantee of the proposed algorithm; c.f. \cite{clash} for more information. A major challenge of using elaborate structure models is the development of efficient projection operators using ideas from combinatorial optimization which is part of ongoing research. 

Mention why we need structured sparsity: applications

\subsubsection{Combinatorial models}

\begin{itemize}
\item Knapsack models
\item Group models
\item Dispersive models
\item Hierarchical models
\end{itemize}

\subsubsection{Convex approaches}

Convexifications and mixed norms.

\subsubsection{Algorithms}



Mention what algorithms are out there: Model-based CS, structured convex norms. Talk about computational issues.

\subsection{Related work}
Tong Zhang's coding complexity method \& greedy algorithm?

==> dispersive_exp.tex <==
\subsection{Neuronal spike detection from compressed data}

In the experiments that follow, we compare the performance of the following three optimization criteria, assuming the dispersive model $\constraint$. 
\begin{equation}
	\begin{aligned}
	& \underset{\x \in \R^\dim}{\text{minimize}}
	& & f(\x)
	& \text{subject to} 
	&& \x \in \constraint.  ~~\quad \quad \quad \quad \quad \quad \quad \quad 
	\end{aligned} \label{eq:disp_discrete} \tag{Discrete model}
\end{equation}

\begin{equation}
	\begin{aligned}
	& \underset{\x \in \R^\dim}{\text{minimize}}
	& & f(\x) + \lambda\cdot \Omega_{\text{exclusive}}(\x).   \quad \quad \quad \quad \quad \quad
	\end{aligned} \label{eq:disp_exclusive} \tag{Exclusive convex norm}
\end{equation}  

\begin{equation}
	\begin{aligned}
	& \underset{\x \in \R^\dim}{\text{minimize}}
	& & \Omega_{\text{exclusive}}(\x)
	& \text{subject to} 
	&& f(\x) \leq \sigma^2. 
	\end{aligned} \label{eq:disp_basis} \tag{Model-based Basis pursuit}
\end{equation}  


\noindent \textbf{Empirical performance on synthetic data:} We first perform experiments on synthetic data. We consider two problem cases: $(i)$ signal denoising from noisy measurements $\obs = \x^{\star} + \noise$, $(ii)$ the CS problem for signal recovery from limited number of linear measurements. 
% to further highlight the strengths and weaknesses of the various sparse dispersive models.

\medskip
\noindent \textit{Signal denoising:} Figure \ref{fig:dispersive1} demonstrates the utility of each approach. For this case, we generate trains of spikes $\x^{\star} \in \R^{\dim}$, where $n = 500$, $\|\x^{\star}\|_0 = 25$ and $\Delta^{\star} = 20$. Without loss of generality and for illustration, we assume $\left(\x^{\star}\right)_i \geq 0, ~\forall i$. In a noisy environment, we observe $\obs = \x^{\star} + \noise$ with $\|\noise\|_2 \leq 10^{-2}$; cf. Figure \ref{fig:dispersive1a}. 

To exploit the dispersive nature of the signal, we use the three approaches described above to reconstruct $\x^{\star}$ for $f(\x) := \frac{1}{2} \|\obs - \x\|_2^2$. In the discrete case, we relax the refractory period $\Delta$ to allow model discrepancies; here, we assume $\Delta = 15$. The denoised signal is shown in Figure \ref{fig:dispersive1b}. Due to $\constraint$, the recovered signal $\widehat{\x}$ is forced to maintain distances between spikes and is composed from a limited number of nonzero coefficients. The solver is based on \cite{baraniuk2010model, needell2009cosamp}.

In contrast to the discrete case, the convex approaches relax $\constraint$; such relaxations are usually apparent in the returned solution. Here, $\widehat{\x}$ dissatisfies $\constraint$ in both Model-based Basis pursuit approach \cite{chen1998atomic} and the exclusive norm-regularized criterion \cite{zhou2010exclusive}; both approaches are solved with best precision using the CVX frameowkr and the SDPT3 solver. For the Model-based Basis pursuit case, $\sigma = 10^{-2}$ while in the regularized exclusive norm case, we set $\lambda = 0.5$. As can be observed in Figures \ref{fig:dispersive1c}-\ref{fig:dispersive1d}, $\widehat{\x}$ identifies the ``strong'' peaks of $\x^{\star}$ but the presence of noise introduces additional spikes in-between, which does not comply with the model and degrades the recovery quality. We underline that in this case, the discrete model shows the best performance on average in terms of the approximation error $\|\widehat{\x} - \x^{\star}\|_2$.
 
\begin{figure}[!ht]
\centering
		\begin{subfigure}[b]{0.49\textwidth}
                \includegraphics[width=1\textwidth]{figs/syn_denoise-crop} 
                \caption{Original signal accoroding to $\constraint$ and the noisy observed signal.}
                \label{fig:dispersive1a}
        \end{subfigure}
		\begin{subfigure}[b]{0.49\textwidth}
                \includegraphics[width=1\textwidth]{figs/syn_dispersive_discrete-crop}
                \caption{Reconstruction using the discrete model and the CoSaMP approach \cite{needell2009cosamp}.}
                \label{fig:dispersive1b}
        \end{subfigure} \\ \medskip
		\begin{subfigure}[b]{0.49\textwidth}
                \includegraphics[width=1\textwidth]{figs/syn_dispersive_exclusive-crop} 
                \caption{Reconstruction using the exclusive norm-regularized convex approach.}
                \label{fig:dispersive1c}
        \end{subfigure}
		\begin{subfigure}[b]{0.49\textwidth}
                \includegraphics[width=1\textwidth]{figs/syn_dispersive_bp-crop} 
                \caption{Reconstruction using the Model-based Basis pursuit.}
                \label{fig:dispersive1d}
        \end{subfigure} 
\caption{\label{fig:dispersive1} Signal de-noising using the dispersive model. Figure \ref{fig:dispersive1a}(Top) depicts the original signal $\x^{\star} \in \R^{500}$ with $\|\x^{\star}\|_0 = 25$ and $\Delta = 20$. We observe $\obs = \x^{\star} + \noise$ with $\|\noise\|_2 \leq 10^{-2}$ as in Figure \ref{fig:dispersive1a}(Bottom). Figures \ref{fig:dispersive1b}-\ref{fig:dispersive1d} illustrate the performance of three approaches: $(i)$ projected gradient descent over the discrete model, $(ii)$ exclusive convex norm regularization and, $(iii)$ model-based basis pursuit.}
\end{figure}

\medskip
\noindent \textit{CS signal recovery:} Figure \ref{fig:dispersive2} illustrates the utility of each approach in the compressed sensing setting where $f(\x) := \frac{1}{2} \|\obs -\sensing\x\|_2^2$. That is, we observe $\x^{\star}$ through a limited set of linear sketches $\obs = \sensing \x^{\star} + \noise \in \R^\numsam$ where $ \sensing \in \R^{\numsam \times \dim}$ is a known linear sketch matrix. Here, we assume $n = 500$ and $m = 70$ for $\|\x^{\star}\|_0 = 25$. The signal $\x^{\star}$ follows the same model as in the previous experiment. 

Figure \ref{fig:dispersive2} indicates the potential performance gains of using each of the proposed criteria. The discrete model \cite{baraniuk2010model, needell2009cosamp} clearly outperforms the rest of the approaches under comparison; such behavior is observed on average. This indicates that the discrete model usually requires fewer measurements for accurate recovery compared to conventional sparse approximation, as long as the underlying signal approximately follows $\constraint$. On the other hand, due to convex relaxations, convex approaches introduce unnecessary nonzero coefficients that do not comply with the underlying model. However, both approaches show good performance in recovering $\x^{\star}$ from limited measurements.

\begin{figure}[!ht]
\centering
		\begin{subfigure}[b]{0.31\textwidth}
                \includegraphics[width=1.1\textwidth]{figs/syn_dispersiveCS_discrete-crop} 
                \caption{}
                \label{fig:dispersive2a}
        \end{subfigure} \hspace{0.25cm}
		\begin{subfigure}[b]{0.31\textwidth}
                \includegraphics[width=1\textwidth]{figs/syn_dispersiveCS_exclusive-crop} 
                \caption{}
                \label{fig:dispersive2b}
        \end{subfigure} \hspace{-0.1cm}
		\begin{subfigure}[b]{0.31\textwidth}
                \includegraphics[width=1\textwidth]{figs/syn_dispersiveCS_bp-crop} 
                \caption{}
                \label{fig:dispersive2c}
        \end{subfigure}
\caption{\label{fig:dispersive2} Performance of dispersive model-based spike train recovery from a limited set of linear measurements. Here, the ambient dimension of $\x^{\star}$ is $n = 500$ while the number of measurements are restricted to $ m =$ for sparsity level $\|\x^{\star}\|_0 = $. (\textbf{Left panel:}) Discrete model recovery. (\textbf{Middle panel:}) Exclusive norm-regularized approach. (\textbf{Right panel:}) Model-based Basis pursuit approach.}
\end{figure}

\medskip
\noindent \textbf{Real neuronal spike data:} In order to understand the functioning of the human brain, it is necessary to identify and study the behavior of neuronal cell membranes under rapid change in the electric potential. However, to observe such phenomena, electrical activities on neurons need to be recorded using specialized equipment. In this experiment, we perform somatic spike detection of a tufted L5 pyramidal cell responding to in-vivo-like current injected in the apical dendrites and the soma simultaneously \cite{incf}. Parasagittal brain slices of the somato-sensory cortex were prepared from $28$-$35$ days-old Wistar rats. Slices were cut in ice-cold extracellular solution (ACSF), incubated at 34 Celsius degrees for 20 minutes and stored at room temperature \cite{naud2009spike}. For more information about the settings of the experiments, we refer the reader to \cite{incf}.

A snapshot of the neuronal spikes waveforms is shown in Figure \ref{fig:neuronal1}. However, to robustly detect the neuronal spikes, a high-frequency sample acquisition equipment is required. Within this context, we apply CS ideas to decrease the number of samples required to approximately detect the \emph{positions} of the spike train. Let $\x^{\star} \in \R^{\dim}$ represent the signal in Figure \ref{fig:neuronal1a}; furthermore, let $\sensing \in \R^{\numsam}$ be the sensing matrix where $\numsam = 0.25 \cdot \dim$, i.e., we perform a $75\%$ compression. 

We use the proposed schemes to recover the locations of the neuronal spikes under the assumption of the dispersive model with refractory period $\Delta$. Here, $\Delta$ is set equal to the \emph{average} period between two consecutive spikes, as observed in practice. 

Figure \ref{fig:neuronal1b} represents the recovered $\sparsity$-sparse approximation using the discrete model $\constraint$. Here, $\sparsity$ is set to the number of spikes expected to appear for a given time period---such number can be easily deduced by observing the behavior of a specific neuron type. From Figure \ref{fig:neuronal1b}, one can easily observe that the discrete model approximates the locations of the spikes quite accurately: most of the spike locations are exactly recovered. However, due to the ``strictness'' of the discrete model, we observe that small deviations from the model assumed lead to imprecise estimations; e.g., between the $12^{\text{th}}$ and $13^{\text{th}}$ spike of the sequence, a larger (than usual) refractory period is observed that leads to mis-location of the next spike estimation.

Figures \ref{fig:neuronal1c}-\ref{fig:neuronal1d} depict the performance of convex solvers using the exclusive norm as $(i)$ regularizer and $(ii)$ objective function. Tweaking the $\lambda$ parameter in the $(i)$ case, one can achieve \emph{sparse} solutions that approximate the underlying model (\ref{fig:neuronal1c}); however, one can observe multiple detected spikes with distance $<\Delta$, i.e., the model is not followed exactly. In the model-based Basis pursuit case, the solver tries to \emph{fit} the solution to the data, which usually leads to less sparse solutions (\ref{fig:neuronal1d}).

We underline that, in the discrete case, the solver searches for a $\sparsity$-sparse signal. In contrast, the convex case usually \emph{fits} the solution into the observations, leading to less sparse solutions. To avoid this inefficiency of the convex norms, we further sparsify the convex solutions in Figures \ref{fig:neuronal1e}-\ref{fig:neuronal1f}. For this problem setup, we observe that even the sparsified solutions violate the dispersive model: the convex norms force the solution to \emph{satisfy} the observations by including more than one spike per true spike location.


\begin{figure}[!h]
\centering
		\begin{subfigure}[b]{0.49\textwidth}
                \includegraphics[width=1\textwidth]{figs/neuronal-crop} 
                \caption{Original neuronal spike train signal.}
                \label{fig:neuronal1a}
        \end{subfigure}
		\begin{subfigure}[b]{0.49\textwidth}
                \includegraphics[width=1\textwidth]{figs/neuronal_discrete-crop}
                \caption{Spike detection using the discrete model.}
                \label{fig:neuronal1b}
        \end{subfigure} \\ \medskip
		\begin{subfigure}[b]{0.49\textwidth}
                \includegraphics[width=1\textwidth]{figs/neuronal_exclusive-crop} 
                \caption{Spike detection using the exclusive norm-regularized convex approach.}
                \label{fig:neuronal1c}
        \end{subfigure}
		\begin{subfigure}[b]{0.49\textwidth}
                \includegraphics[width=1\textwidth]{figs/neuronal_bp-crop} 
                \caption{Spike detection using the Model-based Basis pursuit.}
                \label{fig:neuronal1d}
        \end{subfigure} \\ \medskip
		\begin{subfigure}[b]{0.49\textwidth}
                \includegraphics[width=1\textwidth]{figs/neuronal_exclusive_sparse-crop} 
                \caption{$\sparsity$-sparse approximation of the exclusive norm-regularized convex solution.}
                \label{fig:neuronal1e}
        \end{subfigure}
		\begin{subfigure}[b]{0.49\textwidth}
                \includegraphics[width=1\textwidth]{figs/neuronal_bp_sparse-crop} 
                \caption{$\sparsity$-sparse approximation of the model-based Basis pursuit solution.}
                \label{fig:neuronal1f}
        \end{subfigure}         
\caption{\label{fig:neuronal1} Spike detection in real neuronal data using the dispersive model. Figure \ref{fig:neuronal1a} depicts the original signal $\x^{\star}$. We observe $\obs = \sensing \x^{\star}$ using only $25\%$ measurements through a linear sketch $\sensing$. Figures \ref{fig:dispersive1b}-\ref{fig:dispersive1d} illustrate the performance of the three approaches under comparison. Figures \ref{fig:neuronal1e}-\ref{fig:neuronal1f} show the convex solutions, sparsified to be $\sparsity$-sparse.}
\end{figure}

==> experiments_cluster.tex <==
We perform a compressive sensing experiment to higlight the differences between solutions of \eqref{eq:main} and its convexifications. We take dimensionality reducing measurements of a structured sparse $\x$ via $\mathbf{A}$ and then seek to minimize $f(\x) = \frac{1}{2} \|\y - \A\x\|_2^2$ with a regularizer matched to the structure of $\x$. Our linear measurements $\mathbf{A}$ are randomly subsampled Fourier coefficients of $\x$, and hence, the Lipschitz constant of $f$ is $L=0.5$. 

We compare the performance of three regularizers as summarized in Table \ref{tab:reg}. Since the Ising model \eqref{eq:ising} by itself yields the least squares solution, we add a cardinality constraint to promote sparsity. The new regularizer is still submodular, and its convexification is the sparse total variation regularizer, i.e., the TV semi-norm plus the $\ell_1$-norm. We also include the total variation regularizer alone to emphasize that its solutions are significantly different from  regularization with the Ising model directly.

We consider the standard Shepp-Logan phantom image of size $256 \times 256$ pixels. The resulting image is sparse ($K = 8084$ non-zero pixels) with its coefficients forming constant value clusters, see Fig.\ \ref{fig:shepp}(left). This image suits the TV models that encourage the signal coefficients to have constant values. We then randomly flip the signs of the coefficients, obtaining the {\em Dirty} phantom, Fig.\ \ref{fig:shepp}(right). In this case, the TV models can enforce an incorrect structure as the true coefficient values are not smooth. However, the sign change does not affect the IC penalty, since it is agnostic to the coefficients values and only cares about whether they cluster.
%model is only concerned if a pixel is non-zero, but not to its actual value. since the clusters do not have constant values, 

We show recovery performance using $m = 1.5K$ samples, which is less than the theoretically minimum number of samples for $\ell_0$ recovery (i.e., $m = 2K$). Hence, without the structured sparsity model, it is impossible to do tractable guaranteed recovery. 
We measure performance with the relative recovery error, $E = \|\widehat{\x} - \x\|_2^2/\|\x\|_2^2$, where $\widehat{\x}$ is the estimated image and $\x$ the original one.
The regularization parameters $\lambda$ and $\tau$ have been tuned according to $E$ to yield the best possible result for each model.
The convex models might not yield exactly sparse solutions due to numerical issues. To level the playing field in favor of the convexifications, we  adopt the debiasing heuristic of finding the support of the coefficients that are greater in magnitude than a threshold. We do this by visually inspecting the histogram of the solutions. The debiased estimate is then given by the least squares solution on the  estimated support.
Fig.\ \ref{fig:PhantomRec} presents the recovered images for the original and {\em Dirty} phantom respectively, while Table \ref{tab:res} contains the relative recovery errors.
In the figures, we use the log scale of the coefficients' absolute value to accentuate the errors. 

The debiased estimates perform well in recovering the standard  image, while the TV and TV + L1 penalties fail to set the background exactly to zero. 
Our method recovers the image with no need for debiasing since it correctly identifies the support of the signal. 
It is important to note that in the original phantom, the values of the pixels inside the eyes of the phantom are not exactly zero. Hence the Ising model actually perfectly recovers the entire support. As expected, on the Dirty Shepp-Logan, TV does not perform well. Debiasing helps in this case too, but it is not able to recover the correct support. We also note that our algorithm converges with 4 to 5 iterations, while TV and TV + L1 require thousands of iterations, because the proximal operator of TV cannot be computed in closed form.

==> referenc.tex <==
%%%%%%%%%%%%%%%%%%%%%%%% referenc.tex %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% sample references
% %
% Use this file as a template for your own input.
%
%%%%%%%%%%%%%%%%%%%%%%%% Springer-Verlag %%%%%%%%%%%%%%%%%%%%%%%%%%
%
% BibTeX users please use
% \bibliographystyle{}
% \bibliography{}
%
\biblstarthook{References may be \textit{cited} in the text either by number (preferred) or by author/year.\footnote{Make sure that all references from the list are cited in the text. Those not cited should be moved to a separate \textit{Further Reading} section or chapter.} The reference list should ideally be \textit{sorted} in alphabetical order -- even if reference numbers are used for the their citation in the text. If there are several works by the same author, the following order should be used: 
\begin{enumerate}
\item all works by the author alone, ordered chronologically by year of publication
\item all works by the author with a coauthor, ordered alphabetically by coauthor
\item all works by the author with several coauthors, ordered chronologically by year of publication.
\end{enumerate}
The \textit{styling} of references\footnote{Always use the standard abbreviation of a journal's name according to the ISSN \textit{List of Title Word Abbreviations}, see \url{http://www.issn.org/en/node/344}} depends on the subject of your book:
\begin{itemize}
\item The \textit{two} recommended styles for references in books on \textit{mathematical, physical, statistical and computer sciences} are depicted in ~\cite{science-contrib, science-online, science-mono, science-journal, science-DOI} and ~\cite{phys-online, phys-mono, phys-journal, phys-DOI, phys-contrib}.
\item Examples of the most commonly used reference style in books on \textit{Psychology, Social Sciences} are~\cite{psysoc-mono, psysoc-online,psysoc-journal, psysoc-contrib, psysoc-DOI}.
\item Examples for references in books on \textit{Humanities, Linguistics, Philosophy} are~\cite{humlinphil-journal, humlinphil-contrib, humlinphil-mono, humlinphil-online, humlinphil-DOI}.
\item Examples of the basic Springer style used in publications on a wide range of subjects such as \textit{Computer Science, Economics, Engineering, Geosciences, Life Sciences, Medicine, Biomedicine} are ~\cite{basic-contrib, basic-online, basic-journal, basic-DOI, basic-mono}. 
\end{itemize}
}

\begin{thebibliography}{99.}%
% and use \bibitem to create references.
%
% Use the following syntax and markup for your references if 
% the subject of your book is from the field 
% "Mathematics, Physics, Statistics, Computer Science"
%
% Contribution 
\bibitem{science-contrib} Broy, M.: Software engineering --- from auxiliary to key technologies. In: Broy, M., Dener, E. (eds.) Software Pioneers, pp. 10-13. Springer, Heidelberg (2002)
%
% Online Document
\bibitem{science-online} Dod, J.: Effective substances. In: The Dictionary of Substances and Their Effects. Royal Society of Chemistry (1999) Available via DIALOG. \\
\url{http://www.rsc.org/dose/title of subordinate document. Cited 15 Jan 1999}
%
% Monograph
\bibitem{science-mono} Geddes, K.O., Czapor, S.R., Labahn, G.: Algorithms for Computer Algebra. Kluwer, Boston (1992) 
%
% Journal article
\bibitem{science-journal} Hamburger, C.: Quasimonotonicity, regularity and duality for nonlinear systems of partial differential equations. Ann. Mat. Pura. Appl. \textbf{169}, 321--354 (1995)
%
% Journal article by DOI
\bibitem{science-DOI} Slifka, M.K., Whitton, J.L.: Clinical implications of dysregulated cytokine production. J. Mol. Med. (2000) doi: 10.1007/s001090000086 
%
\bigskip

% Use the following (APS) syntax and markup for your references if 
% the subject of your book is from the field 
% "Mathematics, Physics, Statistics, Computer Science"
%
% Online Document
\bibitem{phys-online} J. Dod, in \textit{The Dictionary of Substances and Their Effects}, Royal Society of Chemistry. (Available via DIALOG, 1999), 
\url{http://www.rsc.org/dose/title of subordinate document. Cited 15 Jan 1999}
%
% Monograph
\bibitem{phys-mono} H. Ibach, H. L\"uth, \textit{Solid-State Physics}, 2nd edn. (Springer, New York, 1996), pp. 45-56 
%
% Journal article
\bibitem{phys-journal} S. Preuss, A. Demchuk Jr., M. Stuke, Appl. Phys. A \textbf{61}
%
% Journal article by DOI
\bibitem{phys-DOI} M.K. Slifka, J.L. Whitton, J. Mol. Med., doi: 10.1007/s001090000086
%
% Contribution 
\bibitem{phys-contrib} S.E. Smith, in \textit{Neuromuscular Junction}, ed. by E. Zaimis. Handbook of Experimental Pharmacology, vol 42 (Springer, Heidelberg, 1976), p. 593
%
\bigskip
%
% Use the following syntax and markup for your references if 
% the subject of your book is from the field 
% "Psychology, Social Sciences"
%
%
% Monograph
\bibitem{psysoc-mono} Calfee, R.~C., \& Valencia, R.~R. (1991). \textit{APA guide to preparing manuscripts for journal publication.} Washington, DC: American Psychological Association.
%
% Online Document
\bibitem{psysoc-online} Dod, J. (1999). Effective substances. In: The dictionary of substances and their effects. Royal Society of Chemistry. Available via DIALOG. \\
\url{http://www.rsc.org/dose/Effective substances.} Cited 15 Jan 1999.
%
% Journal article
\bibitem{psysoc-journal} Harris, M., Karper, E., Stacks, G., Hoffman, D., DeNiro, R., Cruz, P., et al. (2001). Writing labs and the Hollywood connection. \textit{J Film} Writing, 44(3), 213--245.
%
% Contribution 
\bibitem{psysoc-contrib} O'Neil, J.~M., \& Egan, J. (1992). Men's and women's gender role journeys: Metaphor for healing, transition, and transformation. In B.~R. Wainrig (Ed.), \textit{Gender issues across the life cycle} (pp. 107--123). New York: Springer.
%
% Journal article by DOI
\bibitem{psysoc-DOI}Kreger, M., Brindis, C.D., Manuel, D.M., Sassoubre, L. (2007). Lessons learned in systems change initiatives: benchmarks and indicators. \textit{American Journal of Community Psychology}, doi: 10.1007/s10464-007-9108-14.
%
%
% Use the following syntax and markup for your references if 
% the subject of your book is from the field 
% "Humanities, Linguistics, Philosophy"
%
\bigskip
%
% Journal article
\bibitem{humlinphil-journal} Alber John, Daniel C. O'Connell, and Sabine Kowal. 2002. Personal perspective in TV interviews. \textit{Pragmatics} 12:257--271
%
% Contribution 
\bibitem{humlinphil-contrib} Cameron, Deborah. 1997. Theoretical debates in feminist linguistics: Questions of sex and gender. In \textit{Gender and discourse}, ed. Ruth Wodak, 99--119. London: Sage Publications.
%
% Monograph
\bibitem{humlinphil-mono} Cameron, Deborah. 1985. \textit{Feminism and linguistic theory.} New York: St. Martin's Press.
%
% Online Document
\bibitem{humlinphil-online} Dod, Jake. 1999. Effective substances. In: The dictionary of substances and their effects. Royal Society of Chemistry. Available via DIALOG. \\
http://www.rsc.org/dose/title of subordinate document. Cited 15 Jan 1999
%
% Journal article by DOI
\bibitem{humlinphil-DOI} Suleiman, Camelia, Daniel C. O'Connell, and Sabine Kowal. 2002. `If you and I, if we, in this later day, lose that sacred fire...´': Perspective in political interviews. \textit{Journal of Psycholinguistic Research}. doi: 10.1023/A:1015592129296.
%
%
%
\bigskip
%
%
% Use the following syntax and markup for your references if 
% the subject of your book is from the field 
% "Computer Science, Economics, Engineering, Geosciences, Life Sciences"
%
%
% Contribution 
\bibitem{basic-contrib} Brown B, Aaron M (2001) The politics of nature. In: Smith J (ed) The rise of modern genomics, 3rd edn. Wiley, New York 
%
% Online Document
\bibitem{basic-online} Dod J (1999) Effective Substances. In: The dictionary of substances and their effects. Royal Society of Chemistry. Available via DIALOG. \\
\url{http://www.rsc.org/dose/title of subordinate document. Cited 15 Jan 1999}
%
% Journal article by DOI
\bibitem{basic-DOI} Slifka MK, Whitton JL (2000) Clinical implications of dysregulated cytokine production. J Mol Med, doi: 10.1007/s001090000086
%
% Journal article
\bibitem{basic-journal} Smith J, Jones M Jr, Houghton L et al (1999) Future of health insurance. N Engl J Med 965:325--329
%
% Monograph
\bibitem{basic-mono} South J, Blass B (2001) The future of modern genomics. Blackwell, London 
%
\end{thebibliography}

